A Blackbox Approach to Best of Both Worlds in Bandits and Beyond

Best-of-both-worlds algorithms for online learning which achieve near-optimal regret in both the adversarial and the stochastic regimes have received growing attention recently. Existing techniques often require careful adaptation to every new problem setup, including specialised potentials and careful tuning of algorithm parameters. Yet, in domains such as linear bandits, it is still unknown if there exists an algorithm that can simultaneously obtain $O(\log(T))$ regret in the stochastic regime and $\tilde{O}(\sqrt{T})$ regret in the adversarial regime. In this work, we resolve this question positively and present a general reduction from best of both worlds to a wide family of follow-the-regularized-leader (FTRL) and online-mirror-descent (OMD) algorithms. We showcase the capability of this reduction by transforming existing algorithms that are only known to achieve worst-case guarantees into new algorithms with best-of-both-worlds guarantees in contextual bandits, graph bandits and tabular Markov decision processes.

==> backup-data-dependent.tex <==

\section{Data-Dependent Bounds} 
\begin{proof}\textbf{of \pref{thm: basic corral thm} (data-dependent)\quad }
    Define $b_t=B_t-B_{t-1}$. Notice that we have 
    \begin{align*}
        \eta_t \barq_{t,2}b_t &\leq 2\eta_t q_{t,2}b_t \\ 
        &\leq \eta_t q_{t,2} \left(\frac{\frac{c_1\xi_{t}\ind[i_{t}=2]}{q_{t,2}^2} }{\sqrt{c_1\sum_{\tau=1}^{t-1} \frac{\xi_\tau\ind[i_\tau=2]}{q_{\tau,2}^2}}} \right)+ c_2\left(\frac{1}{\min_{\tau\leq t}q_{\tau,2}} - \frac{1}{\min_{\tau\leq t-1}q_{\tau,2}}\right)\\
        &\leq \eta_t \sqrt{c_1} + \eta_t c_2 \left(1-\frac{\min_{\tau\leq t }q_{\tau,2}}{\min_{\tau\leq t-1 }q_{\tau,2}}\right) \\
        &\leq 1. 
    \end{align*}
    By standard analysis for optimistic FTRL (proven in \pref{lem: FTRL}), we have for any $u$,  
    \begin{align*}
        &\sum_{t=1}^{t'} \left(\left\langle \barq_t - u, z_t \right\rangle - (\barq_{t,2} - u_2) b_t\right) \\
        &\leq \sum_{t=1}^{t'} \left(\frac{1}{\eta_{t}} - \frac{1}{\eta_{t-1}}\right)(\psi(u)-\psi(\barq_t)) +  \sum_{t=1}^{t'} \max_q \left(\left\langle \barq_{t} - q, z_t - y_t - \begin{bmatrix}0 \\ b_t \end{bmatrix} \right\rangle  - \frac{1}{\eta_t}D_{\psi}(q, q_t)\right) \\
        &\leq \sum_{t=1}^{t'} \left(\frac{1}{\eta_{t}} - \frac{1}{\eta_{t-1}}\right)(\psi(u)-\psi(\barq_t)) + \sum_{t=1}^{t'} \eta_t \min_{\theta} \left( \barq_{t,1}^{2}\left(z_{t,1}-y_{t,1}-\theta\right)^2 +  \barq_{t,2}^{2}\left(z_{t,2}-y_{t,2}- b_t -\theta\right)^2\right)  \\
        &\leq \frac{\psi(u)}{\eta_{t'}} + 4\sum_{t=1}^{t'} \eta_t \min_{\theta} \left( q_{t,1}^{2}\left(z_{t,1}-y_{t,1}-\theta\right)^2 + q_{t,2}^{2}\left(z_{t,2}-y_{t,2} - b_t - \theta\right)^2\right)
    \end{align*} 
    Rearranging, we get 
    \begin{align*}
        \sum_{t=1}^{t'} \langle q_t - u, z_t\rangle 
        &\leq \underbrace{\frac{\psi(u)}{\eta_{t'}}}_{\term_1} + \underbrace{4\sum_{t=1}^{t'} \eta_t \min_{\theta} \left( q_{t,1}^{2}\left(z_{t,1}-y_{t,1}-\theta\right)^2 + q_{t,2}^{2}\left(z_{t,2}-y_{t,2} - b_t - \theta\right)^2\right)}_{\term_2} \\
        &\qquad + \underbrace{\sum_{t=1}^{t'}\inner{q_t- \barq_t, z_t}}_{\term_3} + \underbrace{\sum_{t=1}^{t'}\barq_{t,2}b_t}_{\term_4} - \underbrace{\sum_{t=1}^{t'}u_2b_t}_{\term_5}
    \end{align*}
    \begin{align*}
        \term_1 
        &\leq \sqrt{\frac{c_1\sum_{t=1}^{t'-1}\sum_{i=1}^2 (\ind[i_t=i]-q_{t,i})^2(\ell_{t,A_t}-m_{t,A_t})^2 + (c_1+c_2^2)\log T}{\log T}}\log T \\
        &\leq \sqrt{c_1\sum_{t=1}^{t'}\sum_{i=1}^2 (\ind[i_t=i]-q_{t,i})^2(\ell_{t,A_t}-m_{t,A_t})^2\log T} + (\sqrt{c_1}+c_2)\log T. 
    \end{align*}
    \begin{align*}
        &\E\left[\term_2\right] \\ &\leq \E\left[\sum_{t=1}^{t'} \eta_t \left(\min_{\theta}\sum_{i=1}^2 q_{t,i}^{2}\left(z_{t,i}-y_{t,i} - \theta\right)^2 + q_{t,2}^2b_t^2\right)\right] \\
        &\leq \E\left[\sum_{t=1}^{t'} \eta_t \min_{\theta}\sum_{i=1}^2 q_{t,i}^{2}\left(z_{t,i}-y_{t,i} - \theta\right)^2 + \sum_{t=1}^{t'} q_{t,2}b_t\right] \\
        &= \E\left[\sum_{t=1}^{t'}\eta_t  \min_{\theta}\sum_{i=1}^2 q_{t,i}^{2}\left(z_{t,i}-y_{t,i} - \theta\right)^2  \right] + \E\left[\sum_{t=1}^{t'} q_{t,2}b_t\right] \\
        &\leq \E\left[ \sum_{t=1}^{t'}\eta_t\min_{\theta}\left(q_{t,1}^2\left(\frac{(\ell_{t,\hatx}-m_{t,\hatx})\ind[i_t=1]}{q_{t,1}}-\theta\right)^2 + q_{t,2}^2\left(\frac{(\ell_{t,\tildeA_t}-m_{t,\tildeA_t})\ind[i_t=2]}{q_{t,2}}-\theta\right)^2 \right) \right] \\
        &\qquad \qquad + \E\left[ \sum_{t=1}^{t'}q_{t,2}b_t \right] \\
        &\leq  \E\left[\sum_{t=1}^{t'}\eta_t\sum_{i=1}^2 (\ind[i_t=i]-q_{t,i})^2(\ell_{t,A_t}-m_{t,A_t})^2\right] + \E\left[\sum_{t=1}^{t'}q_{t,2}b_t \right] \\
        &\leq \E\left[\sqrt{c_1\sum_{t=1}^{t'}\sum_{i=1}^2 (\ind[i_t=i]-q_{t,i})^2(\ell_{t,A_t}-m_{t,A_t})^2\log T}\right] + \E\left[\sum_{t=1}^{t'}q_{t,2}b_t \right]. %\\
        %&\leq \sqrt{\frac{\E\left[\sum_{t=1}^{t'} q_{t,2}\right]\log T}{c_1}} + \E\left[\sum_{t=1}^{t'}q_{t,2}b_t \right]. 
    \end{align*}
    We will further deal with $\sum_t q_{t,2}b_t$ when we bound $\term_4$. 
    \begin{align*}
        \E\left[\term_3\right] = \E\left[ \sum_{t=1}^{t'}\inner{q_t-\barq_t, \E_t[z_t]} \right] = \E\left[ \sum_{t=1}^{t'}\left\langle-\frac{1}{2t^2}\barq_t + \frac{1}{4t^2}\one, \E_t[z_t]\right\rangle \right]\leq O(1). 
    \end{align*}
    \allowdisplaybreaks
    \begin{align*}
            \term_4 &\leq 
            2\sum_{t=1}^{t'}q_{t,2}b_t \\
            &=\sum_{t=1}^{t'} q_{t,2}\left(\frac{\frac{c_1\xi_t\ind[i_t=2]}{q_{t,2}^2}}{\sqrt{c_1\sum_{\tau=1}^t \frac{\xi_\tau\ind[i_\tau=2]}{q_{\tau,2}^2}}}+c_2\left(\frac{1}{\min_{\tau\leq t}q_{\tau,2}}  - \frac{1}{\min_{\tau\leq t-1 }q_{\tau,2}}\right)\right) \\
            &=\sqrt{c_1}\sum_{t=1}^{t'} \sqrt{\frac{\frac{\xi_t\ind[i_t=2]}{q_{t,2}^2}}{\sum_{\tau=1}^{t} \frac{\xi_\tau\one[i_\tau=2]}{q_{\tau,2}^2}}}\times\sqrt{\xi_t\ind[i_t=2]} + c_2\sum_{t=1}^{t'} \left(1-\frac{\min_{\tau\leq t}q_{\tau,2}}{\min_{\tau\leq t-1}q_{\tau,2}}\right)  \\
            &\leq  \sqrt{c_1} \sqrt{\sum_{t=1}^{t'}\frac{\frac{\xi_t\ind[i_t=2]}{q_{t,2}^2}}{\sum_{\tau=1}^{t} \frac{\xi_\tau\one[i_\tau=2]}{q_{\tau,2}^2}}}\times\sqrt{\sum_{t=1}^{t'}\xi_t\ind[i_t=2]} + c_2 \sum_{t=1}^{t'}\log\left(\frac{\min_{\tau\leq t-1}q_{\tau,2}}{\min_{\tau\leq t}q_{\tau,2}}\right)    \tag{Cauchy-Schwarz}\\ 
            &\leq  \sqrt{c_1}\sqrt{1+\log\left(\sum_{t=1}^{t'}\frac{\xi_t\ind[i_t=2]}{q_{t,2}^2}\right)}\sqrt{ \sum_{t=1}^{t'}\xi_t\ind[i_t=2]} + c_2 \log \frac{1}{\min_{\tau\leq t'}q_{\tau,2}} \\
            &\leq \sqrt{c_1\sum_{t=1}^{t'} \xi_t\ind[i_t=2] \log T } + c_2\log T. 
    \end{align*}
    \begin{align*}
        \term_5 = -u_2 B_{t'}  = -u_2\left( \sqrt{c_1\sum_{t=1}^{t'} \frac{\xi_t\ind[i_t=2]}{q_{t,2}^2}} + \frac{c_2}{\min_{t\leq t'} q_{t,2}}\right). 
    \end{align*}
    Overall, we can bound $\E\left[\sum_{t=1}^{t'} \langle q_t - u, z_t\rangle\right] \leq \sum_{j=1}^5 \E[\term_j]$. For comparator $\hatx$, we choose $u=\mathbf{e}_1$ and get 
    \begin{align}
        &\E\left[\sum_{t=1}^{t'} (\ell_{t,A_t} - \ell_{t,\hatx})\right]=\E\left[\sum_{t=1}^{t'} \langle q_t - \mathbf{e}_1, z_t\rangle\right] \nonumber \\
        &\leq \E\left[\sqrt{c_1\sum_{t=1}^{t'}\sum_{i=1}^2 (\ind[i_t=i]-q_{t,i})^2(\ell_{t,A_t}-m_{t,A_t})^2\log T} + \sqrt{c_1\sum_{t=1}^{t'} \xi_t\ind[i_t=2] \log T } \right]+ (\sqrt{c_1}+c_2)\log T.  \label{eq: data dependent tmp}
    \end{align}
    For comparator $x\in\calX\backslash\{\hatx\}$, 
    we choose $u=\mathbf{e}_2$ and bound $\E\left[\sum_{t=1}^{t'} (\ell_{t,A_t} - \ell_{t,\tildeA_t})\right]$ similar as above, with an extra negative term $\term_5$. Again, this cancels the positive part of $\E\left[\sum_{t=1}^{t'}(\ell_{t,\tildeA_t} - \ell_{t,x})\right]$ for $x\in\calX\backslash\{\hatx\}$. At the end, we can bound $\E\left[\sum_{t=1}^{t'} (\ell_{t,A_t} - \ell_{t,x})\right]$ as the right-hand side of \eqref{eq: data dependent tmp}. 
    %\begin{align*}
    %    \E\left[\sum_{t=1}^{t'} (\ell_{t,A_t} - \ell_{t,\tildeA_t})\right] \leq \E\left[\sqrt{c_1\sum_{t=1}^{t'}q_{t,2}\log T} + (\sqrt{c_1}+c_2)\log T\right] - \E\left[ \sqrt{c_1\sum_{t=1}^{t'} \frac{1}{q_{t,2}}} + \frac{c_2}{\min_{t\leq t'} q_{t,2}}\right]. 
    %\end{align*}
    %Combining this with the assumption for the base algorithm on $\E\left[\sum_{t=1}^{t'}(\ell_{t,\tildeA_t} - \ell_{t,x})\right]$, we get that for any $x\in\calX\backslash\{\hatx\}$, 
    %\begin{align*}
    %    \E\left[\sum_{t=1}^{t'}(\ell_{t,A_t} - \ell_{t,x})\right] \leq \E\left[\sqrt{c_1\sum_{t=1}^{t'}q_{t,2}\log T} + (\sqrt{c_1}+c_2)\log T\right].
    %\end{align*}
    %Therefore, it is candidate-aware algorithm with constants $(c_1, \sqrt{c_1}+c_2)$. 
\end{proof}
